Quasi-Isometry Invariance of discrete Higher Filling Functions

We prove that homological filling functions over a ring $R$ equipped with the discrete norm are quasi-isometry invariants for all groups of type $\mathrm{FP}_n$. This confirms a conjecture of Bader-Kropholler-Vankov in the case of discrete norms. The proof uses a technique of equipping free chain complexes with a geometric structure, allowing for analogues of cellular constructions in the purely algebraic setting. As a further application we prove quasi-isometry invariance for a weighted version of integral and discrete filling functions originally introduced in the study of the rapid decay property.

==> preamble.tex <==
% LTeX: enabled=false
\RequirePackage[l2tabu, orthodox]{nag}
\usepackage[dvipsnames]{xcolor}
\usepackage{amsmath, amsthm, amsfonts, mathtools, tikz-cd, amssymb}
\usepackage{enumitem, comment}

% For robustly overwriting macros
\usepackage{letltxmacro}

% Tikz
\usepackage{tikz}
\usepackage{quiver}
\usetikzlibrary{positioning}
\usetikzlibrary{decorations.markings}
\tikzset{
    double line with arrow/.style args={#1,#2}{
        decorate,decoration={markings,%
            mark=at position 0 with {\coordinate (ta-base-1) at (0,1pt);
                \coordinate (ta-base-2) at (0,-1pt);},
            mark=at position 1 with {\draw[#1] (ta-base-1) -- (0,1pt);
                \draw[#2] (ta-base-2) -- (0,-1pt);
            }
        }
    }
}
\tikzset{Equal/.style={-,double line with arrow={-,-}}}

% Fonts and Typography
\usepackage{babel}
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{lmodern}
\usepackage[babel,
    protrusion=true,
    expansion=true,
    kerning=true,
    tracking=true,
    % spacing=true,
]{microtype}
\SetTracking{encoding={*}, shape=sc}{20} % Decrease tracking for smallcaps
\newcommand*{\mathup}[1]{\mathrm{#1}}

\AddToHook{cmd/tableofcontents/before}{%
    \microtypesetup{protrusion=false}
}
\AddToHook{cmd/tableofcontents/after}{%
    \microtypesetup{protrusion=true}
}

% Avoid lines breaks when theorems start with lists
\usepackage{needspace}
\newcommand*{\AvoidPageBreak}{\Needspace*{0pt}}

% Avoid linebreaks in e.g. $n$-connected
\usepackage[shortcuts]{extdash}

% Avoid windows and orphans
\usepackage[all]{nowidow}
\usepackage{csquotes}
% Footnotes punctuation
\usepackage{fnpct}
\mathtoolsset{mathic=true}

%https://tex.stackexchange.com/questions/3490/bad-spacing-of-math-letters-within-italic-text
\def\Noic{\mbox{}\kern-\scriptspace }
\def\noic{\sb{}\kern-\scriptspace }

% (hyper)ref setup
\usepackage[
    pagebackref,
    urlcolor=black,
    linkcolor=blue,
    citecolor=Green,
    allbordercolors=blue,
    citebordercolor=Green
]{hyperref}
\hypersetup{hypertexnames=true}

\usepackage[
    alphabetic,
    backrefs,
    msc-links
]{amsrefs}
\usepackage[thmtools-compat]{keytheorems}

% https://tex.stackexchange.com/questions/565493/link-a-theorem-to-its-restatable
\newkeytheoremstyle{linkedrestate}{%
    headformat={%
        \protect\IfRestatingTF{%
            \protect\hypertarget{orig-#1-#2}{}%
            \protect\hyperlink{restated-#1-#2}{\NAME\thmnumber{ #2}}%
            \NOTE%
        }{%
            \protect\hypertarget{restated-#1-#2}{}%
            \NAME\thmnumber{ #2}%
            \NOTE%
        }%
    },
}

\usepackage{zref-clever}
\zcsetup{
    cap,
    nameinlink,
    abbrev=true,
    countertype={
        defn=definition,
        thm=theorem,
        prop=proposition,
        lem=lemma,
        cor=corollary,
        rem=remark
    }
}
% https://github.com/gusbrs/zref-clever/issues/44
\zcsetup{lastsep = {,~and\nobreakspace}}
\zcRefTypeSetup{condenumi}{
    Name-sg = Condition ,
    name-sg = condition ,
    Name-pl = Conditions ,
    name-pl = conditions ,
    cap = false
}

\AtBeginDocument{\renewcommand{\ref}[1]{\zcref[noname]{#1}}}
\newcommand{\cref}[2][]{\zcref[#1]{#2}}
\newcommand{\lccref}[2][]{\zcref[#1,cap=false]{#2}}
\newcommand{\Cref}[2][]{\zcref[S,#1]{#2}}
\newcommand{\lcnamecref}[2][]{\zcref[noref,nameinlink=false,cap=false,#1]{#2}}

%theorems
\theoremstyle{definition}
\newtheorem{defn}{Definition}[section]
\newtheorem{example}[defn]{Example}
\newtheorem{question}[defn]{Question}
\newtheorem*{question*}{Question}
\newtheorem*{conjecture*}{Conjecture}
\newtheorem{rem}[defn]{Remark}
\newtheorem{convention}[defn]{Convention}
\theoremstyle{plain}
\theoremstyle{linkedrestate}
\newtheorem{thm}[defn]{Theorem}
\newtheorem{lem}[defn]{Lemma}
\newtheorem{prop}[defn]{Proposition}
\newtheorem{cor}[defn]{Corollary}

\numberwithin{equation}{section}

\newlist{condenum}{enumerate}{1}
\setlist[condenum]{label=\upshape(\roman*)}
\setlist[enumerate]{font=\upshape}

\newlist{refenum}{enumerate}{2}
\zcsetup{
    counterresetby = {
        refenumii  = refenumi ,
        refenumiii = refenumii ,
        refenumiv  = refenumiii ,
    }
}
\newcommand{\RefEnumSetCounter}[1]{%
    \setlist[refenum,1]{label=\upshape(\arabic*),ref=\csname the#1\endcsname \,\upshape(\arabic*)}%
    \setlist[refenum,2]{label=\upshape(\alph*), ref=\csname the#1\endcsname \,\upshape(\arabic{refenumi}-\alph*)}%
}
\newcommand{\RefEnumPatchCounterType}[1]{%
    \expanded{%
        \noexpand\zcsetup{%
            countertype = {
                refenumi   = #1 ,
                refenumii  = #1 ,
                refenumiii = #1 ,
                refenumiv  = #1 ,
            }}%
    }%
}

\ExplSyntaxOn
\NewDocumentCommand \IfRefenumCounter { m m m }{
    \str_case:enTF {#1} {
        {refenumi} {}
        {refenumii} {}
        {refenumiii} {}
        {refenumiv} {}
    }{#2}{#3}
}
\ExplSyntaxOff

\makeatletter
\AddToHook{env/refenum/begin}[refenumPatch]{%
    \IfRefenumCounter{\@currentcounter}{%
        % Do nothing. Inherit from parent.
    }{%
        \edef\refenum@parentcounter{\@currentcounter}%
        \edef\refenum@parenttype{\zref@getcurrent{zc@type}}%
        \RefEnumSetCounter{\refenum@parentcounter}%
        \RefEnumPatchCounterType{\refenum@parenttype}%
    }
}
\DeclareHookRule{env/refenum/begin}{refenumPatch}{before}{*}
\makeatother

% Local ref command
% https://tex.stackexchange.com/a/750236/399102
\ExplSyntaxOn
\cs_new_protected:Nn \gaussler_extract_subref:n {
    \__gaussler_extract_last:n #1
}
\cs_new:Nn \__gaussler_extract_last:n {
    \__gaussler_extract_last:w #1 () \q_stop
}
\cs_generate_variant:Nn \gaussler_extract_subref:n {e}
\cs_new:Npn \__gaussler_extract_last:w #1 (#2) #3 \q_stop {
    \tl_if_empty:nTF {#2} {\textbf{??}} {(#2)}
}
\NewDocumentCommand{\localref}{m}{
    \hyperref[#1]{ \textup { \gaussler_extract_subref:e { \getrefnumber{#1} } } }
}
\ExplSyntaxOff

% Symbols
\newcommand{\bbA}{\mathbb{A}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\bbZ}{\mathbb{Z}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbH}{\mathbb{H}}

\newcommand{\bfG}{\mathbf{G}}
\newcommand{\bfH}{\mathbf{H}}
\newcommand{\bfP}{\mathbf{P}}
\newcommand{\bfN}{\mathbf{N}}
\newcommand{\bfM}{\mathbf{M}}
\newcommand{\bfA}{\mathbf{A}}
\newcommand{\bfS}{\mathbf{S}}
\newcommand{\bfT}{\mathbf{T}}
\newcommand{\bfZ}{\mathbf{Z}}

\newcommand{\scrC}{\mathscr{C}}
\newcommand{\scrR}{\mathscr{R}}
\newcommand{\scrH}{\mathscr{H}}
\newcommand{\scrS}{\mathscr{S}}
\newcommand{\scrM}{\mathscr{M}}
\newcommand{\scrN}{\mathscr{N}}
\newcommand{\scrZ}{\mathscr{Z}}

\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calP}{\mathcal{P}}

\newcommand{\calF}{\mathcal{F}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calZ}{\mathcal{Z}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calM}{\mathcal{M}}

% https://tex.stackexchange.com/questions/292047/unicode-math-and-redefine-a-built-in-math-command
\AtBeginDocument{
    \renewcommand{\epsilon}{\varepsilon}
    \renewcommand{\emptyset}{\varnothing}

    \LetLtxMacro{\smalltilde}{\tilde}
    \renewcommand{\tilde}[1]{\widetilde{#1}}
    \LetLtxMacro{\smallhat}{\hat}
    \renewcommand{\hat}[1]{\widehat{#1}}

    \LetLtxMacro{\oldxrightarrow}{\xrightarrow}
    \RenewDocumentCommand{\xrightarrow}{s o m}{%
        \IfBooleanTF{#1}{%
            \oldxrightarrow[#2]{#3}%
        }{%
            \IfValueTF{#2}{%
                \oldxrightarrow[\smash[b]{#2}]{\smash[b]{#3}}
            }{%
                \oldxrightarrow[]{\smash[b]{#3}}
            }%
        }%
    }
}

% General math commands:

\newcommand{\defq}{\coloneqq}
\newcommand{\qdef}{\eqqcolon}

\newcommand{\onto}{\ensuremath\twoheadrightarrow}
\newcommand{\acts}{\curvearrowright}
\newcommand{\commutes}{\text{\Large$\circlearrowleft$}}

\newcommand{\bs}{\backslash}
\newcommand{\cyl}{\operatorname{cyl}}
\newcommand{\cone}{\operatorname*{cone}}
\newcommand{\colim}{\operatorname*{colim}}
\newcommand{\lip}{\mathup{lip}}

\newcommand{\id}{\operatorname{id}}
\newcommand{\im}{\operatorname{im}}
\newcommand{\interior}{\operatorname{int}}
\newcommand{\isom}{\operatorname{Isom}}
\newcommand{\res}{\operatorname{res}}
\newcommand{\ev}{\operatorname{ev}}
\newcommand{\td}{\operatorname{td}}
\newcommand{\cohom}{\operatorname{cohom}}
\newcommand{\vol}{\operatorname{vol}}
\newcommand{\mass}{\operatorname{mass}}
\newcommand{\cd}{\operatorname{cd}}
\newcommand{\rank}{\operatorname{rank}}

\newcommand{\map}{\operatorname{map}}
\newcommand{\pr}{\operatorname{pr}}

\newcommand{\supp}{\operatorname{supp}}

\newcommand{\coker}{\operatorname{coker}}

\newcommand{\homo}{\operatorname{hom}}
\newcommand{\Stab}{\operatorname{Stab}}
\newcommand{\SL}{\operatorname{SL}}
\newcommand{\Fix}{\operatorname{Fix}}
\newcommand{\I}{\operatorname{Im}}
\NewDocumentCommand{\fhom}{E{^}{{}}}{%
    \hom^{\mathup{c}#1}%
}

\newcommand{\PSL}{\operatorname{PSL}}
\newcommand{\PGL}{\operatorname{PGL}}
\newcommand{\GL}{\operatorname{GL}}
\newcommand{\OO}{\operatorname{O}}
\newcommand{\SO}{\operatorname{SO}}
\newcommand{\PO}{\operatorname{PO}}
\newcommand{\SU}{\operatorname{SU}}
\newcommand{\Sp}{\operatorname{Sp}}
\newcommand{\aut}{\operatorname{aut}}
\newcommand{\Ind}{\operatorname{Ind}}

\NewDocumentCommand{\FP}{E{_}{{}}}{%
    \mathup{FP}\IfNoValueTF{#1}{}{_{\mkern-2mu#1}}%
}
\NewDocumentCommand{\F}{E{_}{{}}}{%
    \mathup{F}\IfNoValueTF{#1}{}{_{\mkern-2mu#1}}%
}
\newcommand{\FH}{\mathup{FH}}

\makeatletter
\ExplSyntaxOn
\cs_new:Npn \start_is_cs:nTF #1 {
    \tl_if_empty:nTF { #1 }
    { \use_ii:nn }
    {
        \exp_args:Ne \token_if_cs:NTF { \tl_head:n { #1 } }
    }
}
\NewDocumentCommand{\FirstTokenCommandTF}{ m m m }{
    \start_is_cs:nTF { #1 } { #2 } { #3 }
}
\ExplSyntaxOff

\newbox\usefulbox
\newcommand{\getslant}[1]{\strip@pt\fontdimen1 #1}
\newcommand{\fillKern}[1]{%
    \FirstTokenCommandTF{#1}{%
        \mkern-0.5mu
    }{%
        \setbox\usefulbox=\hbox{$\m@th\scriptstyle #1$}%
        \dimen@ \getslant\the\scriptfont\symletters \ht\usefulbox%
        \kern-\dimen@%
    }%
    #1%
}
\makeatother

\newcommand{\fillvolume}[1][]{\operatorname{FV}_{\fillKern{#1}}}
\newcommand{\weightedfillvolume}[1][]{\operatorname{wFV}_{\fillKern{#1}}}
\newcommand{\filling}[2]{\operatorname{FV}_{\fillKern{#1}}^{#2}}
\newcommand{\weightedfilling}[2]{\operatorname{wFV}_{\fillKern{#1}}^{#2}}
\newcommand{\dfilling}[2]{\operatorname{DFV}_{\fillKern#1}^{#2}}
\newcommand{\weighteddfilling}[2]{\operatorname{wDFV}_{\fillKern{#1}}^{#2}}

\newcommand{\altfilling}[3][]{f_{#3}^{#1#2}}
\newcommand{\weightedaltfilling}[2]{\mathup{w}\kern-1pt f_{#2}^{#1}}

\newcommand{\verythinspace}{%
    \ifmmode%
        \mskip0.5\thinmuskip%
    \else%
        \ifhmode%
            \kern0.08334em%
        \fi%
    \fi%
}
\newcommand{\delimiterSpace}{%
    \mathchoice{\verythinspace}{}{}{}%
}

% https://tex.stackexchange.com/questions/117851/adaptively-sized-delimiters-that-dont-go-beyond-the-size-of-bigl-and-bigr
\usepackage{mleftright}
\makeatletter
\newcommand*{\norm}[1]{%
    \if@display%
        \mathord{\@norm{\displaystyle}{\delimiterSpace #1 \delimiterSpace}}%
    \else%
        \mathord{\@norm{}{\delimiterSpace #1 \delimiterSpace}}%
    \fi%
}
\newcommand*{\@norm}[2]{%
    \@autodelimiterpair{#1}{#2}{\lVert}{\rVert}%
}
\newcommand*{\abs}[1]{%
    %\mathpalette\@abs{#1}
    \mathinner{\@abs{}{#1}}%
}
\newcommand*{\@abs}[2]{%
    \@autodelimiterpair{#1}{#2}{\lvert}{\rvert}%
}
\newcommand*{\@autodelimiterpair}[4]{%
    % a := math axis height -> \dimen0
    \sbox0{$#1\vcenter{}$}%
    \dimen0=\ht0 %
    % formula without delimiters -> \box0
    % h := height of formula -> \ht0
    % d := depth of formula -> \dp0
    \sbox0{$#1#2$}%
    % delta := max(h-a, d+a) -> \dimen2
    \dimen2=\dimexpr\ht0-\dimen0\relax
    \dimen4=\dimexpr\dp0+\dimen0\relax
    \ifdim\dimen4>\dimen2 %
        \dimen2=\dimen4 %
    \fi
    % delimiter's total height >= max(floor(delta/500)*f, 2*delta - l)
    %   -> \dimen4
    % f := \delimiterfactor
    % l := \delimitershortfall
    \dimen4 = \dimen2 %
    \divide\dimen4 by 500 %
    \dimen4=\delimiterfactor\dimen4 %
    \dimen6=\dimexpr 2\dimen2 - \delimitershortfall\relax
    \ifdim\dimen6>\dimen4 %
        \dimen4=\dimen6 %
    \fi
    % formula with \Bigl/\Bigr
    \sbox0{$#1\Bigl#3\Bigr#4$}%
    % comparison: Use \mleft/\mright, if \Bigl/\Bigr is larger than needed
    \ifdim\dimexpr\ht0+\dp0\relax>\dimen4 %
        % Case 1: \Bigl/\Bigr is larger than the minimum needed height.
        %   This means that either (\lvert,\rvert) or (\Bigl\lvert,\Bigr\rvert)
        %   provide the smallest delimiter size that meet the minimum height requirement.
        %   Consequently we can have \mleft/\mright choose (they won't pick anything
        %   larger than \Bigl/\Bigr).
        \mleft#3#2\mright#4
    \else
        % Case 2: \Bigl/\Bigr is exactly right or smaller than the required minimum height
        %   => use \Bigl\Bigr
        \Bigl#3#2\Bigr#4
    \fi
}
\makeatother
\newcommand{\placeholder}{\mskip0.75\thinmuskip\cdot\mskip0.75\thinmuskip}
\newcommand{\size}[1]{\abs{#1}}

\NewDocumentCommand{\dnorm}{m E{_}{{}}}{\norm{#1}_{\mathup{d}#2}}
\NewDocumentCommand{\dabs}{m E{_}{{}}}{\abs{#1}_{\mathup{d}#2}}

\newcommand{\Graph}{\operatorname{Gr}}
\newcommand{\Cay}{\operatorname{Cay}}
\newcommand{\connSupp}{\calC}

\makeatletter
\usepackage{faktor}
\newcommand{\quot}[2]{%
    \if@display%
        \faktor{#1}{#2}%
    \else%
        #1/#2%
    \fi%
}
\DeclareRobustCommand*{\mfaktor}[3][]%
{%
    {\mathpalette{\mfaktorImpl}{{#1}{#2}{#3}}}%
}
\newcommand*{\mfaktorImpl}[2]{\mfaktorImplImpl#1#2}
\newcommand*{\mfaktorImplImpl}[4]{
    \settoheight{\faktor@zaehlerhoehe}{\ensuremath{#1#2{#3}}}%
    \settoheight{\faktor@nennerhoehe}{\ensuremath{#1#2{#4}}}%
    \raisebox{-0.5\faktor@zaehlerhoehe}{\ensuremath{#1#2{#3}}}%
    \mkern-4mu\diagdown\mkern-5mu%
    \raisebox{0.5\faktor@nennerhoehe}{\ensuremath{#1#2{#4}}}%
}
\newcommand{\lquot}[2]{%
    \if@display%
        \mfaktor{#1}{#2}%
    \else%
        #2\kern1pt\bs\kern0.5pt#1%
    \fi%
}
\makeatother

% Punctuation in display math mode
\NewDocumentCommand{\mpct}{s m}{%
    \IfBooleanT{#1}{\thinspace}%
    \text{#2}%
}

\endinput
